Effectively Prefetching Remote Memory with Leap

Memory disaggregation over RDMA can improve the performance of memory-constrained applications by replacing disk swapping with remote memory accesses. However, state-of-the-art memory disaggregation solutions still use data path components designed for slow disks. As a result, applications experience remote memory access latency significantly higher than that of the underlying low-latency network, which itself is too high for many applications. In this paper, we propose Leap, a prefetching solution for remote memory accesses due to memory disaggregation. At its core, Leap employs an online, majority-based prefetching algorithm, which increases the page cache hit rate. We complement it with a lightweight and efficient data path in the kernel that isolates each application's data path to the disaggregated memory and mitigates latency bottlenecks arising from legacy throughput-optimizing operations. Integration of Leap in the Linux kernel improves the median and tail remote page access latencies of memory-bound applications by up to 104.04x and 22.62x, respectively, over the default data path. This leads to up to 10.16x performance improvements for applications using disaggregated memory in comparison to the state-of-the-art solutions.

==> discussion.tex <==
\section{Discussion and Future Work}

\paragraph{Fault-Tolerance} 
Our current implementation of {\name} is not resilient to remote failures. 
Adding the fault-tolerance feature in {\name} is a part of our future work. 
We plan exploring replication to multiple machines or use online erasure-coding over multiple remote regions.

\paragraph{Remote Daemon Optimization} 
{\name} is transparent to remote daemon, and it assumes that the remote daemon will not be the bottleneck. 
In our future work, we want to include an optimized remote daemon in our data path with application-specific memory isolation and data locality.


==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

We have implemented {\name} inside Linux kernel v4.4.125 as a separate data path for remote memory alongside the Linux's traditional data path.
To handle page faults through {\name}, we modified only three functions of the kernel's Memory Management unit. 
The \texttt{do\_swap\_page} function under \texttt{mm/memory.c} handles the page-in operation upon a page fault. 
We added only a single line of code: \texttt{log\_access\_history} to notify {\name}'s page access tracker about the page-fault. 
While paging-in, instead of going through the default \texttt{swapin\_readahead}, we re-route it through the prefetcher's \texttt{do\_prefetch} function. 
Prefetch eviction related functions are added inside  \texttt{mm/swap\_state.c}
To perform remote read/write, inside the \texttt{swap\_readpage} and \texttt{swap\_writepage} functions under \texttt{mm/page\_io.c}, we just invoked a function call \texttt{LEAP\_io\_request} to re-direct the request through  {\name}'s remote I/O interface. 
Same goes for the file systems - bypassing the \texttt{generic\_file\_read} and \texttt{generic\_file\_write} functions through the \texttt{LEAP\_io\_request}. 
Except these re-directions, we did not modify any other existing kernel functions. 

The page access tracker, prefetcher, and {\host} has been added as separate control unit. 
It takes only around 300 lines of code to implement the page access tracker, prefetcher, and the eager eviction mechanism.

%For {\host}, we implemented the design principal of Infiniswap's ~\cite{infiniswap} inside the kernel. 
%The {\host} maintains a per CPU core RDMA connection to the remote machines.
%Each of the RDMA connections maintains an individual RDMA dispatch queue where remote read/write requests are staged. 
%All I/O operations (\eg, remote address mapping, RDMA registration, posting/polling) are independent across threads and processed without synchronization. 
%To handle failure in remote machine, {\name} uses replication over different remote machines. 
%If a remote machine fails or gets unreachable the {\host} relies on the rest available replicas. 
%All RDMA read/write use reliable connection, and one-sided RDMA verbs (RDMA READ, WRITE).

